From Mathematics to Abstract Machine: A formal derivation of an executable Krivine machine

This paper presents the derivation of an executable Krivine abstract machine from a small step interpreter for the simply typed lambda calculus in the dependently typed programming language Agda.

==> eptcsdata.tex <==
\providecommand{\firstpage}{163}
\providecommand{\publicationstatus}{J. Chapman and P. B. Levy (Eds.): Fourth Workshop on \\ Mathematically Structured Functional Programming (MSFP 2012).\\
EPTCS 76, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.76.10}{10.4204/EPTCS.76.10}}

